What are the best systems? New perspectives on NLP Benchmarking

In Machine Learning, a benchmark refers to an ensemble of datasets associated with one or multiple metrics together with a way to aggregate different systems performances. They are instrumental in (i) assessing the progress of new methods along different axes and (ii) selecting the best systems for practical use. This is particularly the case for NLP with the development of large pre-trained models (e.g. GPT, BERT) that are expected to generalize well on a variety of tasks. While the community mainly focused on developing new datasets and metrics, there has been little interest in the aggregation procedure, which is often reduced to a simple average over various performance measures. However, this procedure can be problematic when the metrics are on a different scale, which may lead to spurious conclusions. This paper proposes a new procedure to rank systems based on their performance across different tasks. Motivated by the social choice theory, the final system ordering is obtained through aggregating the rankings induced by each task and is theoretically grounded. We conduct extensive numerical experiments (on over 270k scores) to assess the soundness of our approach both on synthetic and real scores (e.g. GLUE, EXTREM, SEVAL, TAC, FLICKR). In particular, we show that our method yields different conclusions on state-of-the-art systems than the mean-aggregation procedure while being both more reliable and robust.

==> poster/framedblocks.tex <==
\makeatletter
\newcommand\beamerboxesframed[2][]{%
  \global\let\beamer@firstlineitemizeunskip=\relax%
  \vbox\bgroup%
  \setkeys{beamerboxes}{upper=block title,lower=block body,width=\textwidth}%
  \setkeys{beamerboxes}{#1}%
  {%
    \usebeamercolor{\bmb@lower}%
    \globalcolorstrue%
    \colorlet{lower.bg}{bg}%
  }%
  {%
    \usebeamercolor{\bmb@upper}%
    \globalcolorstrue%
    \colorlet{upper.bg}{bg}%
  }%
  %
  % Typeset head
  %
  \vskip4bp
  \setbox\bmb@box=\hbox{%
    \begin{minipage}[b]{\bmb@width}%
      \usebeamercolor[fg]{\bmb@upper}%
      #2%
    \end{minipage}}%
  \ifdim\wd\bmb@box=0pt%
    \setbox\bmb@box=\hbox{}%
    \ht\bmb@box=0pt%
    \bmb@prevheight=-4.5pt%
  \else%
    \wd\bmb@box=\bmb@width%
    \bmb@temp=\dp\bmb@box%
    \ifdim\bmb@temp<1.5pt%
      \bmb@temp=1.5pt%
    \fi%
    \setbox\bmb@box=\hbox{\raise\bmb@temp\hbox{\box\bmb@box}}%
    \dp\bmb@box=0pt%
    \bmb@prevheight=\ht\bmb@box%
  \fi%
  \bmb@temp=\bmb@width%
  \bmb@dima=\bmb@temp\advance\bmb@dima by2.2bp%
  \bmb@dimb=\bmb@temp\advance\bmb@dimb by4bp%
  \hbox{%
    \begin{pgfpicture}{0bp}{+-\ht\bmb@box}{0bp}{+-\ht\bmb@box}
      \ifdim\wd\bmb@box=0pt%
        \color{lower.bg}%
      \else%
        \color{upper.bg}%
      \fi%
      \pgfpathqmoveto{-4bp}{-15.2bp}
      \pgfpathlineto{\pgfpoint{-4bp}{-1bp}}
      \pgfpathqcurveto{-4bp}{1.2bp}{-2.2bp}{3bp}{0bp}{3bp}
      \pgfpathlineto{\pgfpoint{\bmb@temp}{3bp}}
      \pgfpathcurveto%
      {\pgfpoint{\bmb@dima}{3bp}}%
      {\pgfpoint{\bmb@dimb}{1.2bp}}%
      {\pgfpoint{\bmb@dimb}{-1bp}}%
      \bmb@dima=-\ht\bmb@box%
      \advance\bmb@dima by-2.5pt%
      \pgfpathlineto{\pgfpoint{\bmb@dimb}{\bmb@dima}}
      %\pgfpathlineto{\pgfpoint{-4bp}{\bmb@dima}} %% add line between title and body
      %\pgfpathclose
      \pgfsetstrokecolor{black} \pgfsetlinewidth{0.7pt}
      \pgfusepath{stroke, fill}
    \end{pgfpicture}%
    \copy\bmb@box%
  }%
  \nointerlineskip%
  \ifdim\wd\bmb@box=0pt
  \else
    \vskip2.4pt%
  \fi%
  \nointerlineskip%
  \setbox\bmb@colorbox=\hbox{{\pgfpicturetrue\pgfsetcolor{lower.bg}}}%
  \setbox\bmb@box=\hbox\bgroup\begin{minipage}[b]{\bmb@width}%
    \vskip2pt%
    \usebeamercolor[fg]{\bmb@lower}%
    \colorlet{beamerstructure}{upper.bg}%
    \colorlet{structure}{upper.bg}%
    %\color{.}%
}

\def\endbeamerboxesframed{%
  \end{minipage}\egroup%
  \wd\bmb@box=\bmb@width%
  \bmb@temp=\dp\bmb@box%
  \advance\bmb@temp by.5pt%
  \setbox\bmb@box=\hbox{\raise\bmb@temp\hbox{\box\bmb@box}}%
  \dp\bmb@box=0pt%
  \bmb@temp=\wd\bmb@box%
  \bmb@dima=\bmb@temp\advance\bmb@dima by2.2bp%
  \bmb@dimb=\bmb@temp\advance\bmb@dimb by4bp%
  \hbox{%
    \begin{pgfpicture}{0bp}{0bp}{0bp}{0bp}
    \pgfsetlinewidth{0.7pt}
      \unhbox\bmb@colorbox%
      \pgfpathmoveto{\pgfpoint{-4bp}{\ht\bmb@box}}
      \pgfpathlineto{\pgfpoint{-4bp}{1bp}}
      \pgfpathqcurveto{-4bp}{-1.2bp}{-2.2bp}{-3bp}{0bp}{-3bp}
      \pgfpathlineto{\pgfpoint{\the\bmb@temp}{-3bp}}
      \pgfpathcurveto%
      {\pgfpoint{\the\bmb@dima}{-3bp}}%
      {\pgfpoint{\the\bmb@dimb}{-1.2bp}}%
      {\pgfpoint{\the\bmb@dimb}{1bp}}%
      {
      \bmb@dima=\ht\bmb@box%
      \pgfpathlineto{\pgfpoint{\bmb@dimb}{\bmb@dima}}
      \pgfsetstrokecolor{black}\pgfusepath{stroke, fill}
      }
    \end{pgfpicture}%
    \box\bmb@box%
  }%
  \vskip2bp%
  \egroup% of \vbox\bgroup
}
\makeatother

\defbeamertemplateparent{blocks}[framed]{block begin,block end,%
  block alerted begin,block alerted end,%
  block example begin,block example end}[1][]
{[#1]}

\defbeamertemplate{block begin}{framed}[1][]
{
  \par\vskip\medskipamount%
  \begin{beamerboxesframed}[upper=block title,lower=block body,#1]%
    {\raggedright\usebeamerfont*{block title}\insertblocktitle}%
    \raggedright%
    \usebeamerfont{block body}%
}
\defbeamertemplate{block end}{framed}[1][]
{\end{beamerboxesframed}\vskip\smallskipamount}

\defbeamertemplate{block alerted begin}{framed}[1][]
{
  \par\vskip\medskipamount%
  \begin{beamerboxesframed}[upper=block title alerted,lower=block body alerted,#1]%
    {\raggedright\usebeamerfont*{block title alerted}\insertblocktitle}%
    \raggedright%
    \usebeamerfont{block body alerted}%
}%
\defbeamertemplate{block alerted end}{framed}[1][]
{\end{beamerboxesframed}\vskip\smallskipamount}

\defbeamertemplate{block example begin}{framed}[1][]
{
  \par\vskip\medskipamount%
  \begin{beamerboxesframed}[upper=block title example,lower=block body example,#1]
    {\raggedright\usebeamerfont*{block title example}\insertblocktitle}%
    \raggedright%
    \usebeamerfont{block body alerted}%
}%
\defbeamertemplate{block example end}{framed}[1][]
{\end{beamerboxesframed}\vskip\smallskipamount}

==> poster/prelude2.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[]{hyperref}       % hyperlinks
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
%\usepackage[dvipsnames]{xcolor}         % colors
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{dsfont}
\usepackage{mathtools}
\usepackage{pgf}
\usepackage{chngpage}
\usepackage{subcaption}
\usepackage[capitalise, noabbrev]{cleveref}
\usepackage{accents}
\usepackage{adjustbox}
\usepackage[lined]{algorithm2e}

\usepackage[scale=1.24]{beamerposter} % Use the beamerposter package for laying out the poster
\usepackage{tikz}
%\usepackage{enumitem}
\usepackage{etoolbox}
\input{framedblocks.tex} 
\setbeamertemplate{blocks}[framed]

\setbeamercolor{block title}{fg=black,bg=white} % Colors of the block titles
\setbeamercolor{block body}{bg=CornflowerBlue!40!Gray!10!} %Change the alert block title colors} % Colors of the body of blocks
\setbeamercolor{block alerted title}{fg=white,bg=dblue!70} % Colors of the highlighted block titles
\setbeamercolor{block alerted body}{fg=black,bg=dblue!10} % Colors of the body of highlighted blocks
% Many more colors are available for use in beamerthemeconfposter.sty
\setbeamercolor{block title example}{fg=black,bg=dblue!10}




\usetheme{confposter} % Use the confposter theme supplied with this template




%-----------------------------------------------------------
% Define the column widths and overall poster size
% To set effective sepwid, onecolwid and twocolwid values, first choose how many columns you want and how much separation you want between columns
% In this template, the separation width chosen is 0.024 of the paper width and a 4-column layout
% onecolwid should therefore be (1-(# of columns+1)*sepwid)/# of columns e.g. (1-(4+1)*0.024)/4 = 0.22
% Set twocolwid to be (2*onecolwid)+sepwid = 0.464
% Set threecolwid to be (3*onecolwid)+2*sepwid = 0.708

\newlength{\sepwid}
\newlength{\onecolwid}
\newlength{\twocolwid}
\newlength{\threecolwid}
\setlength{\paperwidth}{48in} % A0 width: 46.8in
\setlength{\paperheight}{36in} % A0 height: 33.1in
\setlength{\sepwid}{0.024\paperwidth} % Separation width (white space) between columns
\setlength{\onecolwid}{0.22\paperwidth} % Width of one column
\setlength{\twocolwid}{0.464\paperwidth} % Width of two columns
\setlength{\threecolwid}{0.708\paperwidth} % Width of three columns
\setlength{\topmargin}{-0.5in} % Reduce the top margin size
%-----------------------------------------------------------
\usepackage{caption}
\usetikzlibrary{decorations.pathreplacing,calligraphy}

\captionsetup[figure]{labelformat=empty}

\usepackage{graphicx}  % Required for including images

\usepackage{booktabs} % Top and bottom rules for tables

\usetikzlibrary{shapes.misc}
 \usetikzlibrary{calc,matrix}
\tikzset{
  mycross/.pic={
    \draw[pic actions] 
      (-2pt,-2pt) -- (2pt,2pt)
      (-2pt,2pt) -- (2pt,-2pt);
  },
}


\usepackage{tikz-qtree}
\usetikzlibrary{arrows.meta,bending}
\tikzset{every tree node/.style={minimum width=2em,draw,circle},
     blank/.style={draw=none},
     edge from parent/.style=
     {draw, edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}},
     level distance=1.5cm}
\newcommand{\AxisRotator}[1][rotate=0]{%
    \tikz \draw[x=.5em,y=2.25em,line width=.2ex,-stealth,#1] (0,0) arc (-150:150:1 and 3.5);%
    }
\newcommand{\AxisRotatorbis}[1][rotate=0]{%
    \tikz \draw[x=.5em,y=1.25em,line width=.2ex,-stealth,#1] (0,0) arc (-150:150:1 and 5.5);%
}
\definecolor{vert}{rgb}{0,0.4,0.2}
\definecolor{bleu}{rgb}{0.2,0.2,0.7}
\colorlet{rouge}{BrickRed}
\definecolor{gris}{rgb}{0.57, 0.64, 0.69}

\definecolor{grey}{rgb}{0.4,0.4,0.4}
\definecolor{green}{rgb}{0,0.4,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{red}{rgb}{1,0,0}
\definecolor{purple}{rgb}{0.5,0.,0.9}
\definecolor{greydark}{rgb}{0.5,0.5,0.5}


